Spectral Embeddings Leak Graph Topology: Theory, Benchmark, and Adaptive Reconstruction

Graph Neural Networks (GNNs) excel on relational data, but standard benchmarks unrealistically assume the graph is centrally available. In practice, settings such as Federated Graph Learning, distributed systems, and privacy-sensitive applications involve graph data that are localized, fragmented, noisy, and privacy-leaking. We present a unified framework for this setting. We introduce LoGraB (Local Graph Benchmark), which decomposes standard datasets into fragmented benchmarks using three strategies and four controls: neighborhood radius $d$, spectral quality $k$, noise level $\sigma$, and coverage ratio $p$. LoGraB supports graph reconstruction, localized node classification, and inter-fragment link prediction, with Island Cohesion. We propose AFR (Adaptive Fidelity-driven Reconstruction), a method for noisy spectral fragments. AFR scores patch quality via a fidelity measure combining a gap-to-truncation stability ratio and structural entropy, then assembles fragments using RANSAC-Procrustes alignment, adaptive stitching, and Bundle Adjustment. Rather than forcing a single global graph, AFR recovers large faithful islands. We prove heat-kernel edge recovery under a separation condition, Davis--Kahan perturbation stability, and bounded alignment error. We establish a Spectral Leakage Proposition: under a spectral-gap assumption, polynomial-time Bayesian recovery is feasible once enough eigenvectors are shared, complementing AFR's deterministic guarantees. Experiments on nine benchmarks show that LoGraB reveals model strengths and weaknesses under fragmentation, AFR achieves the best F1 on 7/9 datasets, and under per-embedding $(\epsilon,\delta)$-Gaussian differential privacy, AFR retains 75% of its undefended F1 at $\epsilon=2$. Our anonymous code is available at https://anonymous.4open.science/r/JMLR_submission

==> figures/main_figure.tex <==
% === Put this in your preamble if not already present ===
% \usepackage{tikz}
% \usetikzlibrary{positioning,calc,arrows.meta,fit}

\begin{figure}
\centering
\begin{tikzpicture}[>=latex,
    every node/.style={circle, draw, thick, minimum size=7.5mm, inner sep=0pt, font=\small},
    edge/.style={line width=1.0pt},
    miss/.style={edge, dashed}
]

% Colors for subgraphs
\colorlet{Cyc}{blue!65}
\colorlet{Star}{green!65!black}
\colorlet{Path}{orange!85!black}
\colorlet{Kfour}{red!70!black}

% --------------------------------------------------------
% Top-Left: 4-cycle (diamond)
% --------------------------------------------------------
\node[fill=Cyc] (c0) at (-3.0,  2.0) {0};
\node[fill=Cyc] (c1) at (-2.0,  3.0) {1};
\node[fill=Cyc] (c2) at (-1.0,  2.0) {2};
\node[fill=Cyc] (c3) at (-2.0,  1.0) {3};

\draw[edge, Cyc] (c0) -- (c1) -- (c2) -- (c3) -- (c0);
% Optional diagonal for a different look:
%\draw[edge, Cyc] (c1) -- (c3);

% --------------------------------------------------------
% Top-Right: star (center + 3 leaves)
% --------------------------------------------------------
\node[fill=Star] (s0) at ( 3.0,  2.0) {4}; % center
\node[fill=Star] (s1) at ( 4.2,  2.0) {6};
\node[fill=Star] (s2) at ( 3.8,  3.2) {7};
\node[fill=Star] (s3) at ( 3.8,  0.8) {5};

\draw[edge, Star] (s0) -- (s1);
\draw[edge, Star] (s0) -- (s2);
\draw[edge, Star] (s0) -- (s3);

% --------------------------------------------------------
% Bottom-Left: path of length 3 (4 nodes)
% --------------------------------------------------------
\node[fill=Path] (p0) at (-3.0, -2.0) {8};
\node[fill=Path] (p1) at (-2.0, -2.0) {9};
\node[fill=Path] (p2) at (-1.0, -2.0) {10};
\node[fill=Path] (p3) at ( 0.0, -2.0) {11};

\draw[edge, Path] (p0) -- (p1) -- (p2) -- (p3);

% --------------------------------------------------------
% Bottom-Right: K4 (complete graph on 4 nodes)
% --------------------------------------------------------
\node[fill=Kfour] (k0) at ( 2.2, -3.0) {12};
\node[fill=Kfour] (k1) at ( 3.2, -1.8) {15};
\node[fill=Kfour] (k2) at ( 4.2, -3.0) {13};
\node[fill=Kfour] (k3) at ( 3.2, -4.2) {14};

% All edges of K4
\foreach \a/\b in {k0/k1,k0/k2,k0/k3,k1/k2,k1/k3,k2/k3}{
  \draw[edge, Kfour] (\a) -- (\b);
}

% --------------------------------------------------------
% Missing inter-subgraph links to be predicted (dashed)
% --------------------------------------------------------
\draw[miss] (c1) -- (s0);   % top-left cycle to star center
\draw[miss] (s1) -- (p1);   % star leaf to path
\draw[miss] (p3) -- (k1);   % path end to K4 node
\draw[miss] (p2) -- (k3);   % path start to K4 node
\draw[miss] (p1) -- (c0);
\draw[miss] (s3) -- (k1);
\draw[miss] (k0) -- (c2);

% --------------------------------------------------------
% Labels (optional): subgraph titles
% --------------------------------------------------------
\node[draw=none, fill=none, font=\footnotesize] at (-2.0,  3.6) {Cycle subgraph};
\node[draw=none, fill=none, font=\footnotesize] at ( 3.4,  3.8) {Star subgraph};
\node[draw=none, fill=none, font=\footnotesize] at (-2.0, -2.6) {Path subgraph};
\node[draw=none, fill=none, font=\footnotesize] at ( 3.2, -4.8) {$K_{4}$ subgraph};

% Legend (minimal)
\draw[miss] (-3.0, -4.8) -- (-2.0, -4.8);
\node[draw=none, fill=none, anchor=west, font=\footnotesize] at (-1.5, -4.8)
    {Missing link};

\end{tikzpicture}
\caption{An illustration of the fragmented graph scenario in LoGraB. Four distinct subgraphs are shown: a cycle (top-left), a star (top-right), a path (bottom-left), and a complete graph $K_4$ (bottom-right). Solid edges represent observed intra-subgraph connectivity, while dashed edges indicate missing inter-subgraph links that must be predicted (Task 3: Inter-fragment Link Prediction).}
\label{fig:fragmented_graph}
\end{figure}

